Differential Privacy on Trust Graphs

We study differential privacy (DP) in a multi-party setting where each party only trusts a (known) subset of the other parties with its data. Specifically, given a trust graph where vertices correspond to parties and neighbors are mutually trusting, we give a DP algorithm for aggregation with a much better privacy-utility trade-off than in the well-studied local model of DP (where each party trusts no other party). We further study a robust variant where each party trusts all but an unknown subset of at most $t$ of its neighbors (where $t$ is a given parameter), and give an algorithm for this setting. We complement our algorithms with lower bounds, and discuss implications of our work to other tasks in private learning and analytics.

==> sections/experiments_forc.tex <==
\section{Experiments}\label{sec:experiments}

% Our experiments supplement the theory by analyzing the error from the proposed protocols on 
We analyze the theoretically proven error bounds on real network datasets. We focus our analysis on two performance aspects: \textit{(i)} the \textit{improvements} over the error that come from applying the notion of TGDP compared to the fully conservative LDP, and \textit{(ii)} the \textit{trade-off} between robustness and efficiency when applying the RTGDP definition. Experiments on real communication and social networks show that the LP protocol (\Cref{thm:lp-protocol}) for achieving TGDP yields a significant reduction in the error bound compared to LDP.  Furthermore, the protocol for achieving RTGDP (\Cref{thm:lp-protocol-robust}) still has markedly lower error than LDP even when a large number of neighbors could be compromised.  

\paragraph*{Datasets.} We analyzed nine network datasets publicly available from the Stanford Large Network Dataset Collection (SNAP) \citep{snapnets}: three email communication datasets, two Bitcoin trust network datasets, and four social network datasets. 
%For directed graphs, we converted directed edges to undirected edges (results may of course change when direction is preserved). 
Individual details about each dataset are given in~\Cref{app:exp}. % TODO (serena): describe each network dataset.

\paragraph*{Implementation.}
Our analysis of the MSE of the proposed protocols focuses on computing $\OPT_{\LP}$ and $\OPT^{\mathbf{t}}_{\LP}$ for each graph.  Code and implementation details for solving these using \texttt{cvxpy} are included in the Supplementary Material \citep{diamond2016cvxpy,agrawal2018rewriting}. 

\subsection{Error: TGDP vs LDP}

We compare the upper bound on the MSE using the mechanism described in~\Cref{thm:lp-protocol}  to that of standard LDP mechanisms~(\Cref{def:int-ldp}).  Specifically, the ($\varepsilon, G$)-TGDP mechanism proposed in Theorem \ref{thm:lp-protocol} achieves an MSE at most $2\Delta^2 \cdot \OPT_{\LP}/\varepsilon^2$ whereas LDP with a classic randomized response mechanism \cite{warner1965randomized} with randomized rounding achieves an error of $\Theta(\Delta^2 n / \varepsilon^2)$.  We refer to the ratio of these quantities, namely, $\frac{\OPT_{\LP}}{n}$, as the \textit{TGDP error ratio} for a given graph.

Table \ref{tab:lp_experiments} shows the TGDP error ratio for all datasets. On the evaluated graph, the TGDP error ratio ranged between $0.002$ and $0.207$, which suggests that the TGDP protocol obtains appreciably reduced MSE.

\begin{table}[!ht]
\caption{TGDP error ratios for 9 network datasets.}
\label{tab:lp_experiments}
% \vskip -0.3in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrrr}
\toprule
Dataset & $n$ & $\OPT_{\LP}$ & $\frac{\OPT_{\LP}}{n}$ \\
\midrule
EU Emails (Core)  & $1,005$ & $111.97$ & $0.111$ \\
EU Emails (All) & $265,214$ & $18,074.40$ & $0.068$  \\
Enron Emails   & $36,692$ & $3,060.66$ & $0.083$  \\
Bitcoin (OTC) & $5,881$ & $1126$ & $0.191$  \\
Bitcoin (Alpha) & $3,783$ & $686$ & $0.181$  \\
Facebook & $4,039$ & $10$ & $0.002$ \\
GitHub & $37,700$ & $4,538$ & $0.120$ \\
Epinions & $75,879$ & $15,734$ & $0.207$  \\
Twitter & $81,306$ & $961$ & $0.012$  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table} 

\subsection{Error of RTGDP}

The RTGDP definition is more conservative than TGDP, especially as the number of untrusted neighbors per node increases. 
%Here, we evaluate how much efficiency is lost in practice for different levels of robustness. 
% We evaluate the error bounds on real networks for the robust trust graph DP protocol as the number of mistrusted nodes varies from $0$ (basic Trust Graph DP) to mistrusting all neighbors. 
To evaluate the trade-off between robustness and error, we compute $\OPT^{\mathbf{t}}_{\LP}$ for varying degrees of mistrust $\mathbf{t}$ for four graphs of size $n < 10,000$. These include one email communication graph, two Bitcoin trust graphs, and one social network graph. For each graph, we vary the degree of mistrust $\mathbf{t}$ as follows:
for each $\alpha$, we construct $\bt_{\alpha} = \lceil \alpha \cdot \bdeg_V \rceil = (\lceil \alpha \cdot \deg(v) \rceil)_{v \in V} $.
Thus, $\alpha$ represents the proportion of neighbors that are untrusted for each node. We then compute $\OPT^{\mathbf{t}_{\alpha}}_{\LP}$ for various $\alpha \in [0,1]$.
As before, we study the \textit{$\mathbf{t}_{\alpha}$-RTGDP error ratio}, $\frac{\OPT^{\mathbf{t}_{\alpha}}_{\LP}}{n}$.

\begin{figure}[!ht]
    \vskip -0.2in
    \centering
    \begin{small}
    \begin{tblr}{p{0.2cm}c}
        \SetCell[r=2]{}$\frac{\OPT^{\mathbf{t}_{\alpha}}_{\LP}}{n}$ & \includegraphics[trim={0 18pt 0 0},clip,width=0.5\columnwidth]{figures/robust_mse.pdf}\\
        & Proportion of untrusted neighbors $\alpha$ \\
    \end{tblr}
    \end{small}
    \caption{$\mathbf{t}_{\alpha}$-RTGDP error ratios for varying proportions of untrusted neighbors $\alpha$ for 4 datasets with $n < 10,000$. }
    \label{fig:robust_lp_experiments}
\end{figure}

Figure \ref{fig:robust_lp_experiments} shows the $\mathbf{t}_{\alpha}$-RTGDP error ratios for varying levels of mistrust $\alpha$. The initial jump in the error ratio at $\alpha=0.1$ comes from the ceiling rounding, which affects all nodes with a single neighbor. Notably, for all datasets, an error ratio of less than $0.6$ can still be achieved for $\alpha$ up to $0.5$. This suggests that the RTGDP notion may be a  practical way to interpolate between LDP and TGDP, as considerable error reductions can still occur for RTGDP for $\alpha < 0.5$.

%In summary, our experiments show that on a number of real communication, trust, and social network datasets, the proposed protocols for Trust Graph DP and Robust Trust Graph DP have upper bounds on error that are appreciably lower than that of Local DP. Thus, further exploration into implementing these notions in practice may result in efficiency gains in otherwise Local DP settings.

==> sections/introduction_old.tex <==
% Previous version of the introduction as of 2/1/24 at 11:15am (moved by Serena)
\section{Introduction}

\emph{Differential privacy} (DP) \cite{dwork2006calibrating, dwork2006our} is a rigorous notion of privacy that has seen extensive study (e.g., \cite{dwork2014algorithmic, vadhan2017complexity}) and widespread adoption in data analytics and machine learning (e.g., \citet{abowd2018us, tf-privacy, pytorch-privacy}). It dictates that the output of a randomized algorithm remains statistically indistinguishable if the data of a single user were to change. The most widely studied models of DP are the \emph{central} model where a trusted curator is given access to the raw data and required to output a DP estimate of the function of interest, and the \emph{local} model \cite{evfimievski2003limiting, kasiviswanathan2011can} where all the messages leaving each user’s device are required to be DP. While the local DP model is very compelling in that each user needs to place minimal trust in other users, it is known to suffer from a significantly higher utility degradation compared to the central DP model.

Real world settings often include situations where a user is willing to put more trust in a different subset of users. This stems from the fact that many people actually have different privacy sensitivities for different people in their lives -- for example, Alice might want to share her location data with family and close friends, but not willing to have her location data be recoverable by strangers from a public mechanism. This is related to the concept of privacy through \textit{control over information}, in that users specify with whom they are willing share their information \citep{solove2002conceptualizing}. 
%Examples include devices belong to the same household or owned by the same company.
Such situations can be captured by a \emph{trust graph} where vertices correspond to different users and neighboring vertices are mutually trusting. In this work, we study DP over such trust graphs, whereby the DP guarantee is enforced on the messages exchanged by each vertex or its trusted neighbors on one hand, and the other non-trusted vertices on the other hand. More precisely, the distribution of all messages exchanged by each vertex $v$ or one of its neighbors with any vertices that are not trusted by $v$ should remain statistically indistinguishable if the input data held by $v$ changes. For a formal definition, we refer the reader to Definition~\ref{???}.

% \begin{definition}[Trust Graph DP]

% \end{definition}

In notion described above, the privacy guarantee can break if a single neighbor of a vertex turns out to be untrustworthy. This leads us to also study the following robust version of the definition.

% \begin{definition}[Robust Trust Graph DP]

% \end{definition}

We give DP algorithms for the basic \emph{aggregation} primitive on both non-robust and robust trust graphs. Specifically, we show that ???.

We complement our algorithms with lower bounds proving that ???.

The aggregation primitive that we study in this work is a basic building block in machine learning and data analytics. Indeed, our work implies new DP algorithms on both non-robust and robust trust graphs for a variety of other problems including ???, ??? and ???.

\subsection{Motivation}
The DP on trust graphs model is an intermediate setting between local and central DP. It allows formalizing a notion of (differential) privacy in cases where users have different privacy levels for different subsets of the population, as well as settings where  users can place different levels of trust on different digital services or sub-platforms. While one can think of different settings where trust graphs naturally arise, we next discuss two particular scenarios:

\paragraph{Social graphs.} In a social network setting where a user’s posts are visible to their friends but hidden from strangers, computing analytics (e.g., histograms of users’s check-ins in different geographic locations) or training a machine learning model (e.g., a generative model on the users’ posted photos) without entrusting a central curator naturally leads to peer-to-peer protocols that are trust graph DP with the trust graph being the social graph.

\paragraph{Consent graphs.}

A user might consent for the data they generate on some online service to be shared in the clear with only a specific set of other services. As each user might have their own consent choices for every pair of services, this induces a bipartite trust graph where on one side each vertex corresponds to a (user, service) pair, and on the other side, each vertex corresponds to a service. The presence of an edge between $(u, A)$ and $B$ then indicates that user $u$ consented for their data on service $A$ to be shared in the clear with service $B$. It might also be acceptable for data to be exchanged between a pair of services even if no consent was provied by the user as long as the exchanged data is anonymous. If DP is deemed to meet the bar for data anonymization, then DP on the bipartite trust graph described above would be a better-suited model than central DP (which would not be acceptable privacy-wise due to the lack of a single service that is allowed to see the data in the clear) or local DP (which would result in an unnecessarily poor utility).

\paragraph{Routing games.} Differentially private routing games \citep{dong2015differential} recommend routes while requiring the origins and destinations of drivers to be considered private. In this more relaxed setting, each driver may be willing to share their origin and destination with a subset of other drivers. This willingness is demonstrated by the location sharing feature on Google maps, where users share their locations with subsets of other users. 
    
\paragraph{Disease contact tracing.} A contact tracing mechanism alerts users if they have been in recent contact with someone who has contracted the disease. Alice is willing to share whether she has a disease directly with her close friends and family, but wants the mechanism to be differentially private with respect to her data in its outputs for strangers. That is, a stranger cannot discover whether or not Alice has the disease given what the mechanism outputs for them. 
    
\paragraph{Personalized shopping recommendations.} An advertisement recommender system provides Alice with recommendations based on her browsing history. However, it is important that strangers are not able to back out Alice's browsing history to through their own recommendations. This is particularly important if Alice's browsing history contains medical information.     In this network-DP version, Alice is actually fine with her personal shopping history being shared with her spouse and affecting her spouse's recommendations, given that they share a household.

\subsection{Technical Overview}

\badih{Do we want to discuss the linear programming approach here?}

\badih{Do we want to discuss the minimum dominating set problem here?}

\paragraph{Organization of the Rest of the Paper.}
We start with some notation and differential privacy preliminaries in Section~\ref{sec:prelim}. In Section~\ref{sec:trust_graph_DP}, we formally define the notion of DP on trust graphs, and give algorithms and a lower bound for solving the aggregation task under this privacy guarantee. The robust trust graph DP notion is defined in Section~\ref{ref:robust_trust_graph_DP} where we also give an algorithm and lower bounds for aggregation under this robust privacy guarantee. We provide the results of a supporting experimental evaluation in Section~\ref{sec:experiments}. We conclude with some interesting future directions in Section~\ref{sec:conc_fut_dir}. In Appendix~\ref{ref:related_work}, we discuss related prior work. Missing proofs are given in Appendix~\ref{app:proofs}. Some experimental details are deferred from the main body to Appendix~\ref{app:exp}.

==> sections/oldtext-agg.tex <==
\section{Aggregation in Graph DP}

\subsection{Extension to Quantile Estimation}

We extend this ``slightly better protocol'' to quantile estimation. Suppose each vertex $v$ has a single data point, $x_v \in \mathbb{R}$. The goal is to find a quantile $q$ over all $n$ vertices. Let $\mathcal{Y}$ be the output space, for which $|\mathcal{Y}| = D < \infty$.

A centralized $\eps$-DP exponential mechanism incurs error of at most $O(\log(D)/\eps)$ by setting utility for a dataset $X$ for quantile $q$ to be $u(X, o) = -\big| |\{x \in \mathcal{X}: x \leq o \}| - qn \big|$ \citep{gillenwater2021differentially, smith2011privacy}.

\begin{corollary}
There is an $(\eps, 0)$-DP mechanism for finding a quantile $q$ with error at most $O(\log(D) \sqrt{OPT_{LP}}/\eps)$ with probability at least $(1-O(\log(D))p)(1-p)$, where $p$ is the error probability from Theorem \ref{thm:lp-protocol}.
\end{corollary}

\begin{proof}[Proof Sketch]
    We can estimate quantile $q$ using the following procedure: For each $y_j \in \mathcal{Y}$, one can run an $\eps_j$-DP sum protocol to query the result of $\sum_{i=1}^n \Ind(x_i \leq y_j)$ (procedure referred to as $SumQuery(y_j, \eps_j)$). By Theorem \ref{thm:lp-protocol}, this query incurs error at most $O(\sqrt{OPT_{LP}}/\eps_j)$ with probability $p$. Suppose we perform binary search and run this query $O(\log(D))$ times. The binary search procedure runs as follows:

\begin{algorithm}
\caption{Binary Search With Error}\label{alg:binsearch}
\begin{algorithmic}
\Require Bounds $L, R$
\State Initialize bounds $L \gets 0$, $R \gets D - 1$.
\State $m \gets \lfloor(L+R)/2\rfloor$
\State $\hat{r}(y_m) \gets SumQuery(y_m, \eps_m)$ \Comment{Assuming $y_m$ has rank $m$ in sorted $\mathcal{Y}$}
\State error $\gets O(\sqrt{OPT_{LP}/\eps_m})$
\If{$|\hat{r}(y_m) - qn| \leq$ error or $L \geq R$} 
    \Return $y_m$
\ElsIf{$\hat{r}(y_m) < qn$ - error}
    \State $BinarySearch(m+1, R)$
\ElsIf{$\hat{r}(y_m) > qn$ + error}
    \State $BinarySearch(L, m-1)$
\EndIf 
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:binsearch} has a probability of failure. 
$\hat{r}(y_m) < qn - \text{error}$ implies that the actual $r(y_m) < qn$ with probability $1-p$. If one of these comparisons is ``bad,'' e.g. $r(y_m) > qn$ when $\hat{r}(y_m) < qn - \text{error}$, then the BinarySearch procedure will overshoot, such that the new $L,R$ interval will not include a value of $y_m$ with $r(y_m) = qn$. It's still possible to recover from this due to the error tolerance, but not guaranteed.


The full procedure will terminate correctly with some $y_m$ that satisfies $|\hat{r}(y_m) - qn| \leq$ error if for all intermediate comparisons, the actual $r(y_m) < qn$ when $\hat{r}(y_m) < qn - \text{error}$ (and the equivalent version for $>$). Applying the union bound, the probability that at least one of the $O(\log(D))$ comparisons is ``bad'' (e.g. $r(y_m) > qn$ when $\hat{r}(y_m) < qn - \text{error}$) is at most $O(\log(D))p$. Other algorithms exist to reduce the final error probability by applying additional comparisons \citep{feige1994computing,rivest1980coping,karp2007noisy}. The true rank is then within $2\sigma$ of $qn$ with probability $1-p$.

Anything that terminates Algorithm \ref{alg:binsearch} will have rank at most $O(\sqrt{OPT_{LP}}/\eps_j)$ away from $qn$ (for the $j$ at which it terminates). Basic composition says that this is now $(\sum_{j=1}^{\log(D)} \eps_j)$-DP. If we set $\eps_j = \frac{\eps}{\log(D)}$, we have that the full error of this $\eps$-DP procedure is $O(\log(D) \sqrt{OPT_{LP}}/\eps)$.
\end{proof}

\subsubsection{Backtracking binary search}

\begin{algorithm}
\caption{Backtracking Binary Search}\label{alg:binsearchbacktrack}
\begin{algorithmic}
\Require Bounds $L, R$, parent bounds $L', R'$, sorted $y_0,...y_{D-1}$, DP parameter $\eps'$
\State Initialize bounds $L \gets 0$, $R \gets D - 1$.
\State $\sigma$ $\gets O(\sqrt{OPT_{LP}/\eps'})$
\State $\hat{r}(y_L) \gets SumQuery(y_L, \eps')$
\State $\hat{r}(y_R) \gets SumQuery(y_R, \eps')$
\If{$|\hat{r}(y_L) - qn| \leq$ $\sigma$} 
    \Return $y_L$ \Comment{Check for termination.}
\ElsIf{$|\hat{r}(y_R) - qn| \leq$ $\sigma$} 
    \Return $y_R$
\EndIf
\If{$\hat{r}(y_L) > qn$  or $\hat{r}(y_R) < qn$}
    \State $BinarySearch(L', R')$ \Comment{Backtrack to previous bounds.}
\EndIf
\State $m \gets \lfloor(L+R)/2\rfloor$ 
\State $\hat{r}(y_m) \gets SumQuery(y_m, \eps')$
\If{$\hat{r}(y_m) < qn$}
    \State $BinarySearch(m+1, R)$ \Comment{Identify next branch to search.}
\ElsIf{$\hat{r}(y_m) > qn$}
    \State $BinarySearch(L, m-1)$
\EndIf 
\end{algorithmic}
\end{algorithm}

Suppose $P(|\hat{r}(y) - r(y)| > \sigma) \leq p$, with $P(\hat{r}(y) > r(y) + \sigma) \leq \frac{p}{2}$ and $P(\hat{r}(y) < r(y) - \sigma) \leq \frac{p}{2}$. That is, we assume that $SumQuery(y, \eps')$ returns an estimated rank $\hat{r}(y)$ within $\sigma$ error of the actual rank $r(y)$ with constant probability $p$. Suppose the error is distributed symmetrically such that $P(\hat{r}(y) > r(y)) = \frac{1}{2}$.

Define $\nu(t) = (L,R)$ to be a node in the binary search tree containing the bounds being checked at round $t$. 
    
Define $W$ to be the set of ``promising nodes'' in which the procedure might likely terminate: $$W = \{ (L,R) : r(y_L) \in [qn - \sigma, qn + \sigma] \text{ or } r(y_R) \in [qn - \sigma, qn + \sigma]\}.$$
\pasin{I don't think the definition above is correct since it doesn't include the setting where $r(y_L) < qn - \sigma$ and $y(y_R) > qn + \sigma$ and $y_R = y_L + 1$ (i.e. the third case in the similar definition in \cite{karp2007noisy})}

\snote{Good point. Here the equivalent ``third case'' would be $R = L+1$ and $qn \in [r(y_L), r(y_R)]$. I removed that third case for simplicity and am assuming that $\mathcal{Y}$ is fine grained enough and $r$ is smooth enough that the max distance between any adjacent $r(y)$'s is no more than $\sigma$. But, the rest of the results should go through if we add back the third case. The main change I think will be to the final error, where now the worst-case error between the answer $r(y)$ and $qn$ has to include the max distance between adjacent $r(y)'s$: $\max_j|r(y_{j+1}) - r(y_j)|$. If $\mathcal{Y}$ includes all possible $x_i$ values in the network, then $\max_j|r(y_{j+1}) - r(y_j)| \leq \max_j|r(x_{j+1}) - r(x_j)|$, which is a cost inherent to quantile estimation. Maybe we can argue that this is constant?}

\begin{lemma}\label{lem:lowskip}
    (Generalization of Lemma 5.2 from \cite{karp2007noisy}) Conditional on the event that $\nu(t) \in W$, the probability that the algorithm halts at time $t$ is at least $1-p$.
\end{lemma}
\begin{proof}
    $\nu(t) \in W$ implies two independent cases: $r(y_L) \in [qn - \sigma, qn + \sigma]$ or $r(y_R) \in [qn - \sigma, qn + \sigma]$. Without loss of generality we consider the first case. If $r(y_L) \in [qn - \sigma, qn]$, then the procedure halts if $\hat{r}(y_L) \in [r(y_L), r(y_L)+ \sigma]$, which happens with probability at least $\frac{1-p}{2}$. Similarly, if $r(y_L) \in [qn, qn + \sigma]$, then the procedure halts if $\hat{r}(y_L) \in [r(y_L) - \sigma, r(y_L)]$ which happens with the same probability at least $\frac{1-p}{2}$. The probability of halting conditioned on $r(y_L) \in [qn - \sigma, qn + \sigma]$ is a convex sum of the individual disjoint cases, so the probability of halting in case 1 is at least $\frac{1-p}{2}$. A similar argument follows for the second case. Overall, $P(\text{halt} | \nu(t) \in W) \leq P(\text{halt} | \text{case 1}) + P(\text{halt} | \text{case 2}) \leq 1-p$.
\end{proof}

\begin{lemma}\label{lem:goodmove}
    (Generalization of Lemma 5.3 from \cite{karp2007noisy}) Conditional on the event that $\nu(t) \notin W$, the probability that $d(\nu(t+1), W) = d(\nu(t), W) - 1$ is at least $(1-\frac{p}{2})^3$.
\end{lemma}
\begin{proof}
Let $(L,R)$ be the value of $\nu(t)$. If  $\nu(t) \notin W$, then one of the following cases applies:
\begin{enumerate}
    \item $[r(y_L), r(y_R)] \subseteq [0, qn - \sigma] \cup [qn + \sigma, n]$, or
    \item $r(y_L) < qn - \sigma$ and $r(y_R) > qn + \sigma$.
\end{enumerate}
In case 1,  either $r(y_L) > qn + \sigma$ or $r(y_R) < qn - \sigma$. Assume $r(y_L) > qn + \sigma$ without loss of generality. Then $P(\hat{r}(y_L) > qn) \geq P(\hat{r}(y_L) > r(y_L) - \sigma) \geq 1 - \frac{p}{2}$. If so, then $\nu(t+1)$ backtracks to the parents of $\nu(t)$, and is closer to $W$ since no descendent of $\nu(t)$ belongs to $W$, so $P(d(\nu(t+1), W) = d(\nu(t), W) - 1 | \text{case 1}) \geq 1 - \frac{p}{2}$.

In case 2, let $E$ denote the event that we do not backtrack. This is equivalent to the event that $\hat{r}(y_L) < qn$ and $\hat{r}(y_R) > qn$. Assuming $r(y_L) < qn - \sigma$, $P(\hat{r}(y_L) > qn) \leq P(\hat{r}(y_L) > r(y_L) + \sigma) \leq \frac{p}{2}$. Therefore, $P(\hat{r}(y_L) < qn) \geq 1 - \frac{p}{2}$. Thus, as the product of the two independent events, $P(E) \geq (1 - \frac{p}{2})^2$.

If $r(y_m) \in [qn - \sigma, qn + \sigma]$, then we are done, as either child node $\nu(t+1) = (L, m)$ or $\nu(t+1)= (m,R)$ will be in $W$. If $r(y_m) \notin [qn - \sigma, qn + \sigma]$, then assume without loss of generality that $r(y_m) < qn - \sigma$. This implies that all of $W$ is contained in the right subtree of $\nu(t)$. $\nu(t+1)$ moves to the right subtree if $\hat{r}(y_m) < qn$. Since we've assumed that $r(y_m) < qn - \sigma$, $P(\hat{r}(y_m) > qn) \leq P(\hat{r}(y_m) > r(y_m) + \sigma) \leq \frac{p}{2}$. Therefore, $\nu(t+1)$ moves to the right subtree with probability at least $1 - \frac{p}{2}$. 

Overall, in case 2, $P(d(\nu(t+1), W) = d(\nu(t), W) - 1 | \text{case 2}) \geq P(E)(1-\frac{p}{2}) \geq (1-\frac{p}{2})^3$.
\end{proof}

\begin{lemma}\label{lem:backtracking_speed}
Suppose $p$ is chosen such that $(1-\frac{p}{2})^3 > \frac{1}{2}$. Then for $t > O(\log{D})$, backtracking binary search terminates in $t$ or more rounds with probability at most $O(e^{-t})$.

\end{lemma}
\begin{proof}
    Adapted from Proposition 5.1 from \cite{karp2007noisy}. 
    
    Let $Y_t = d(\nu(t), W)$, which is shortest distance in the binary search tree between the node $\nu(t)$ and any node in $W$.

    Let $Z_t = |\{s < t | \nu(x) \in W\}|$. This is the number of nodes ``promising nodes'' that were visited before round $t$.

    Let $\Phi_t = \log_2(n) + Z_t - Y_t - \frac{1}{8}(t-Z_t)$. 
    Then $\Phi_t$ is a submartingale, since $\Phi_0 = \log_2(n) - D(\nu(0), W) \geq 0$, and $E[\Phi_{t+1} | \Phi_{t}] > \Phi_t$, which we show below:
    $$E[\Phi_{t+1} | \Phi_{t}] = E[\Phi_{t+1} | \Phi_{t}, \nu(t) \in W]P(\nu(t) \in W) +E[\Phi_{t+1} | \Phi_{t}, \nu(t) \notin W]P(\nu(t) \notin W)$$
    
    If $\nu(t) \in W$, then
    \begin{align*}
        E[\Phi_{t+1} | \Phi_{t}, \nu(t) \in W] = \log_2(n) + Z_t + 1 - E[Y_{t+1}|\Phi_t, \nu(t) \in W] - \frac{1}{8}(t - Z_t)
    \end{align*}
    $Y_{t+1} \leq d(\nu(t), W) + 1$, and $d(\nu(t), W) = 0$; therefore,
    $E[Y_{t+1}|\Phi_t, \nu(t) \in W] \leq 1$
    which implies that $E[\Phi_{t+1} | \Phi_{t}, \nu(t) \in W] \geq \Phi_t$.
    
    If $\nu(t) \notin W$, then $Z_{t+1} = Z_t$, so
    \begin{align*}
        E[Y_{t+1} | Y_t, \nu(t) \notin W] &= E[d(\nu(t+1), W) | d(\nu(t), W), \nu(t) \notin w] \\
        &\leq (d(\nu(t), W) - 1(1-\frac{p}{2})^3 + (d(\nu(t), W) + 1)(1-(1-\frac{p}{2})^3) \\
        &\leq Y_t - (1-2(1-\frac{p}{2})^3) \leq Y_t \text{ since }(1-\frac{p}{2})^3 < \frac{1}{2}.
    \end{align*}
    Therefore, $E[\Phi_{t+1} | \Phi_{t}, \nu(t) \notin W] \geq \Phi_t$.

    Now we show that with high probability, the algorithm terminates after $t < 160(1 + \log_2(n))$ steps. If $t > 160(1 + \log_2(n))$, then either $Z_t > \frac{t}{10}$, or if $Z \leq \frac{t}{10}$, then
    $\Phi_t < \log_2(n) - \frac{t}{80} < \frac{t}{160} - \frac{t}{80} = -\frac{t}{160}$.

    Applying Lemma \ref{lem:lowskip}, $P(Z_t > \frac{t}{10}) = (1-p)^{\frac{t}{10}}$ by just multiplying the probability of the independent events.

    Applying Azuma's inequality in the second case,
    $P(\Phi_t < -\frac{t}{160}) \leq P(\Phi_t < \Phi_0 - \frac{t}{160}) \leq e^{-\frac{t}{320}}$.

    Therefore, the probability that the algorithm terminates after $t > 160(1 + \log_2(D))$ steps is at most $\max((1-p)^{\frac{t}{10}}, e^{-\frac{t}{320}})$. Assuming that $p < 1$ is constant, this is $O(e^{-t})$.
\end{proof}

\begin{corollary}
There is an $(\eps, 0)$-DP mechanism for finding a quantile $q$ with  error at most $O(\log(D) \sqrt{OPT_{LP}}/\eps)$ with probability at least $0.99(1-p)$.
\end{corollary}
\begin{proof}

    Suppose there exists a known finite set $\mathcal{Y}$ which contains the full domain from which the $x_i$'s are drawn. Let $D = |\mathcal{Y}|$.

    Suppose we manually terminate the algorithm at $160(1 + \log_2(D)) + K$ rounds. By Lemma \ref{lem:backtracking_speed}, the probability that we would have to manually terminate the algorithm is
    $$P(t > 160(1 + \log_2(D)) + K) \leq P(t > 160(1 + \log_2(D))) \leq e^{-\frac{t}{C}},$$
    for some constant $C$.
    For $t > 160(1 + \log_2(D)) + K$, we have $$e^{-\frac{t}{C}} < e^{-\frac{160(1 + \log_2(D)) + K}{C}} = e^{-\frac{1}{2}}(\frac{1}{\sqrt{D}})(e^{-\frac{K}{C}}).$$ 
    Setting $K \geq C(-\log(0.01))$ is sufficient to bound this final term by the desired $0.01$. Thus, for the chosen constant $K$, the probability of manually terminating after $160(1 + \log_2(D)) + K$ rounds and receiving a bad answer is at most $0.01$.
    
    If not manually terminated, suppose the algorithm outputs a value $y_i$. Then $|\hat{r}(y_i) - qn| < \sigma$, which implies that $$P(|r(y_i) - qn| > 2\sigma) \leq P(|r(y_i) - \hat{r}(y_i)| + |\hat{r}(y_i) - qn| > 2\sigma) \leq P(|r(y_i) - \hat{r}(y_i)| > \sigma) \leq p.$$
    The probability of receiving a good answer is then $$P(\text{not manually terminated}) \times P(\text{good answer} | \text{not manually terminated}) \geq 0.99(1-p).$$
    \pasin{I'm not sure I understand how the above is derived. In particular, $r(y_i) - \hat{r}(y_i)$ is not just an independent noise any more but the noise \emph{conditioned on termination}. See for example Lemma 5.1 in \cite{karp2007noisy} on how they handle the incorrect probability.}
    
    \snote{Good question! I think this is actually different from Lemma 5.1, which shows that $$P(\text{halt at time }t, \text{bad answer} | \text{termination test performed at time }t) < 4/n.$$ On the other hand, I'm conditioning on halting as well, and trying to measure $P(\text{bad answer} | \text{halt before time }t)$. Specifically, I argue that for the chosen $T = 160(1 + \log_2(D)) + K$, $$P(\text{bad answer}) = P(\text{halt after time } T)(1) + P(\text{halt before time } T)P(\text{bad answer} | \text{halt before time }T).$$
    I am assuming that $P(\text{bad answer} | \text{halt before time }T)$ is independent of $T$, and is just equal to $$P(\text{bad answer} | \text{halt with answer }y) = P(|r(y) - qn| > 2\sigma 
    \;\big|\; |\hat{r}(y) - qn| < \sigma) \leq p.$$ Does that make sense?}

    Any good answer will have rank at most $O(\sqrt{OPT_{LP}}/\eps')$ away from $qn$. If we run Backtracking Binary Search for $T$ iterations, basic composition says that this is now $3T\eps'$-DP. If we set $\eps' = \frac{\eps}{3T}$, we have that the full error of this $\eps$-DP procedure is $O(T \sqrt{OPT_{LP}}/\eps)$. We had previously chosen $T = O(\log(D))$.
\end{proof}

\subsubsection{A simpler question}

A simpler scenario is to consider only the case where just the ``diagonal'' has data. Namely, we have nodes $1, \dots, n$ and $(i, j)$ for all $i, j \in [n]$. Each node $(i, j)$ is connected to both $i$ and $j$ but only the nodes $1, \dots, n$ contains the data $x_1, \dots, x_n$. 

In this case, the upper bound is $O(\sqrt{n} / \eps)$ whereas the lower bound is the trivial $O(1/\eps)$.

\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}
    \node[shape=circle,draw=black] (1) at (0,3) {$x_1$};
    \node[shape=circle,draw=black] (2) at (2,3) {$x_2$};
    \node[shape=circle,draw=black] (3) at (4,3) {$x_3$};
    \node[shape=circle,draw=black] (4) at (6,3) {$x_4$};
    \node[shape=circle,draw=black] (12) at (1,2) {};
    \node[shape=circle,draw=black] (23) at (3,2) {};
    \node[shape=circle,draw=black] (34) at (5,2) {};
    \node[shape=circle,draw=black] (13) at (2,1) {};
    \node[shape=circle,draw=black] (24) at (4,1) {};
    \node[shape=circle,draw=black] (14) at (3,0) {};

    \path [-] (12) edge node[left] {} (1);
    \path [-] (12) edge node[left] {} (2);

    \path [-] (23) edge node[left] {} (2);
    \path [-] (23) edge node[left] {} (3);

    \path [-] (34) edge node[left] {} (3);
    \path [-] (34) edge node[left] {} (4);

    \path [-] (13) edge[bend left] node[left] {} (1);
    \path [-] (13) edge[bend right] node[left] {} (3);

    \path [-] (24) edge[bend left] node[left] {} (2);
    \path [-] (24) edge[bend right] node[left] {} (4);
    
    \path [-] (14) edge[bend left] node[left] {} (1);
    \path [-] (14) edge[bend right] node[left] {} (4);

\end{tikzpicture}
    \caption{Illustration of a graph with a large gap between upper and lower bound error in A.3.1. Each data-containing node shares exactly one neighbor with each other data-containing node.}
    \label{fig:network}
\end{figure}

\paragraph{An even simpler question.} Consider an even simpler scenario where each node $i$ sends their data $x_i$ to the nodes $(i, j)$ for all $j \in [n]$, and the node $(i, j)$ then have to immediately publish some randomized output $f_{i, j}(x_i, x_j)$. Then, the outputs $f_{1, 2}(x_1, x_2), \dots, f_{n-1,n}(x_{n-1}, x_n)$ are then combined to estimate the summation.

This is perhaps the most restrictive protocol possible, i.e. there is not even share randomness among $i, j$ and the communication is truly one round. Nonetheless, we do not know how to prove a lower bound even for this.

One observation (which is not hard to prove) is the following:
\begin{observation}
Suppose that the entire protocol is $\eps$-DP.
Then, for every $i \in [n]$, there exists $\eps^1_i, \dots, \eps^n_i \geq 0$ such that $\sum_{j \in [n]} \eps^j_i \leq 2\eps$ and $f_{i, j}(x_i, x_j)$ is $\eps^j_i$-DP for $x_i$.
\end{observation}
In other words, the privacy guarantee is derived from applying the basic composition theorem (up to a factor of two--which comes from the fact that the privacy loss is not necessary symmetric).

\pasin{Even in this setting, I do not know how to prove a lower bound. I've tried the following ``reduction to local-DP'' approach. First, try to show that if $f_{i, j}(x_i, x_j)$ is $\eps$-DP for both $x_i, x_j$, then it can be viewed as a post-processing of $\eps'$-DP randomized response on $x_i, x_j$. Once this is the case, we basically go back to the local-DP setting and can apply lower bounds from there. Unfortunately, this fails: $\eps'$ can be as large as $\sqrt{\eps}$, which means that we do not get any bound. Interestingly this $\sqrt{\eps}$ bound also seems to be tight as demonstrates by the ``equality'' function where $f_{i, j}(x_i, x_j)$ is the $\eps$-DP randomized response applied on whether $x_i = x_j$; it seems to me that any decomposition of this into two independent randomized responses of $x_i, x_j$ requires $\sqrt{\eps}$-DP.}

\section{Mean Estimation}

In the mean estimation problem, there is an underlying distribution $D$ over $[0, 1]$ and each $x_u$ is draw i.i.d. from $D$. The goal is to output an estimate of the mean of $D$ (under the same network DP definition as before).

We can again formulate an optimization problem for this task if we were to use a similar algorithm as before. Let $w_v \in [0, 1]$ denote the weight of $x_v$ to be included (under the constraint $\sum_{v \in V} w_v = 1$), and $y_v$ the variance of noise added by $v$. That is, the final estimate is of the form $\left(\sum_{v \in V} w_v x_v\right) + Z$ where $Z$ is the noise from DP that has variance $\sum_{v \in V} y_v$. This total estimate has variance at most $\frac{1}{4} \sum_{v \in V} w_v^2 + \sum_{v \in V} y_v$. Therefore, this gives us the following:
\begin{align*} %\label{eq:opt-mean-est}
&\min \frac{1}{4} \sum_{v \in V} w_v^2 + \sum_{v \in V} y_v \\
&\text{s.t.} \sum_{u \in N[v]} y_u \geq w^2_v\left(\frac{2}{\eps^2}\right) &\forall v \in V \\
& \qquad \sum_{v \in V} w_v = 1 \\
& \qquad 0 \leq w_u \leq 1 &\forall u \in V.
\end{align*}
This is a convex problem and can therefore be solved efficiently.

This is equivalent to a second order conic program (SOCP) with the following parameters:

\begin{align*}
    \min_x \quad &f^\top x \\
    \text{s.t.} &||A_0 x + b_0|| \leq c_0^\top x + d_0 \\
    &||A_v x + b_v || \leq c_v^\top x + d_v \text{ for } v \in V \\
    & Fx = g \\
    & 0 \leq y_u, w_u \leq 1 &\forall u \in V \\
\end{align*}

The exact parameters are as follows: 

Let $\bar{0}_{|V|}$ and $\bar{1}_{|V|}$ denote vectors of length $|V|$ of $0$'s and $1$'s, respectively.

Let $\bar{1}_v$ denote a vector of length $|V|$ with $1$ in the $v$'th entry and $0$ otherwise.

Let $\mathbf{0}_{|V|}$ denote a $|V| \times |V|$ matrix of $0$'s. 

Let $I_{|V|}$ a $|V| \times |V|$ identity matrix.

Let $\bar{1}_{N[v]}$ be vector of length $|V|$ with entries of $1$ for indices $u \in N[v]$ and $0$ for all other indices.

\begin{align*}
    &x = [w, y, t] \text{ for } w, y \in \mathbb{R}^{|V|}, t \in \mathbb{R} \\
    &f = [\bar{0}_{|V|}, \bar{1}_{|V|}, 1] \\
    &A_0 = \begin{bmatrix}
    \frac{1}{2} I_{|V|} & \mathbf{0}_{|V|} & 0 \\
    \bar{0}_{|V|} & \bar{0}_{|V|} & 1
    \end{bmatrix}; \quad b_0 = [\bar{0}_{|V|}, 0]; \quad c_0 = [\bar{0}_{|V|}, \bar{0}_{|V|}, 1] \quad d_0 = 1 \\
    &A_v = \begin{bmatrix}
    \frac{\sqrt{2}}{\varepsilon} \bar{1}_{v} & \bar{0}_{|V|} & 0 \\
    \bar{0}_{|V|} & -\bar{1}_{N[v]} & 0
    \end{bmatrix}; \quad b_v = [0, \frac{1}{4}]; \quad c_v = [\bar{0}_{|V|}, \bar{1}_{N[v]}, 0] \quad d_v = \frac{1}{4} \\
\end{align*}

The final box constraints can also be written as second order cone constraints.

% More details on converting between QCQP and SOCP: https://www.zubairkhalid.org/ee563/2020/module2.pdf

\textbf{Relation to summation LP protocol} This mean estimation program can do better than the LP dominating set protocol by a factor of $O(\frac{1}{\eps^2})$. The graph structure that hits this is one where half the nodes form a star, and the other half of the nodes are all unconnected and independent. In the previous dominating set protocol, we would have to add noise for each of the unconnected nodes; whereas this mean estimation protocol allows downweighting these independent nodes.

Pasin postulates that the mean estimation convex program is similar to a partial dominating set problem, and is upper bounded by the max over $t$ of $t-$partial dominating set solutions.

\section{Related work}
\subsection{Personalized federated learning}
Federated learning considers a setting where a centralized model only receives gradients from different individuals. \textit{Personalized} federated learning clusters individuals based on their differing objectives, and allows different individuals to receive different outputs. In the gradient descent process, a different model is essentially learned per cluster.

There is also work in differentially private federated learning. However, as far as I know this has not been combined with personalization, or done in a setting with an individual has different tiers of privacy sensitivity. 

\subsection{Personalization and learning theory}

\subsection{Gossip networks}

\subsection{Heterogenous DP}
We initially consider a setting where all users share a common $\eps$-DP privacy requirement for people other than their children. A more general heterogenous setting could allow different individuals to select different values of $\eps$ for different connections in the network. 


==> sections/robust-old.tex <==

\section{Robust Trust Graph DP}

\subsection{Upper Bound}

Consider the following linear program (LP):
\begin{align*} 
&\min \sum_{s \in S} y_s \\
&\text{s.t.} \sum_{s \in (N[c] \setminus T)} y_s \geq 1 &\forall v \in V, T \in \binom{N(c)}{t_c} \\
& \qquad 0 \leq y_s \leq 1 &\forall s \in S. \nonumber
\end{align*}

When $\bt = \bzero$, this LP coincides with an LP relaxation of the set cover problem (where each server $s$ corresponds to a set and each client $c$ corresponds to an element), and its solution can be smaller than the minimum set cover size by a factor of $O(\log |C|)$.

Before we proceed, we note that the above program \eqref{eq:lp-robust} can have exponential size due to the presence of the constraint \eqref{eq:sum-const} for all $T \in \binom{N(V)}{t_c}$. However, it can still be solved in polynomial time because an efficient separation oracle exists for the group of constraints~\eqref{eq:sum-const}. More specifically, for each $v \in V$, we can check~\eqref{eq:sum-const} by picking letting $T$ be the $t_c$ maximum values and check the inequality for just that $T$ (instead of enumerating over all $T \in \binom{N(c)}{t_c}$).

To describe the protocol, let $\NB(r, p)$ denote the negative binomial with parameters $r, p$. Define $\sNB(r, p)$ as a distribution of $X - X'$ where $X, X' \sim \NB(r, p)$ are i.i.d.

\begin{theorem}\label{thm:lp-protocol}
Let $\optlp^{\bt}$ denote the optimal of LP specified in \Cref{eq:lp-robust}. Then, there is a $\bt$-robust $\eps$-TDP mechanism for binary summation with MSE $O\left(\sqrt{\optlp^{\bt}}/\eps\right)$.
\end{theorem}

\pasin{The protocol below can be easily adapted to real summation by appropriately scaling $x_c$ and $z_s$.}

\begin{proof}[Proof Sketch]
The protocol works as follows:
\begin{itemize}
\item Let $q$ be a sufficiently large number e.g. $q > 2n$.
\item Each client $c \in C$ randomly picks $\{a^s_c\}_{s \in N(c)} \subseteq \Z_q$ uniformly among those that satisfies $\sum_{s \in N[c]} a^s_c = x_c$.
\item Each server $s \in S$, randomly pick $z_s \sim \sNB(y_s, e^{-\eps})$ and publish $z_s + \sum_{c \in N(s)} a^s_c$.
\item The final estimate is the sum of all published numbers (rounded appropriately, i.e. if larger than $q/2$, then round to a negative number by subtracting $q$ from it).
\end{itemize}
The error is simply to analyzed: it is at most the error before moduloing, i.e. $\sum_{u \in V} z_u$ which is distributed exactly as $\sNB\left(\sum_{u \in V} y_u, e^{-\eps}\right)$ whose standard deviation is $O\left(\frac{\sum_{u \in V} y_u}{\eps}\right)$.

As for the privacy, notice that for every $c \in C$ and $T \in \binom{N(c)}{t_c}$, the view $\VIEW^{V \setminus (N[c] \setminus T)}$ that depends on $x_c$ consists only of $\{z_s + a^s_c\}_{s \in (N(c) \setminus T)}$ and $\{a^s_c\}_{s \in T}$. Observe that due to the additive shares, the only information learned about $x_v$ is through the sum of these numbers, i.e. $x_c + \sum_{s \in(N(c) \setminus T)} z_s$ \pasin{The previous two sentences needs to be formalized further.} $\left(\sum_{s \in (N(c) \setminus T)} z_s\right)$ is distributed exactly as $\sNB(\sum_{s \in (N(c) \setminus T)} y_s, e^{-\eps})$. \eqref{eq:sum-const} ensures that $\sum_{s \in (N(c) \setminus T)} y_s \geq 1$; the r.v. $\left(\sum_{s \in (N(c) \setminus T)} z_s\right)$ can thus be viewed as the sum of two independent r.v. $Z \sim \sNB(1, e^{-\eps})$ and $Z' \sim \sNB(\sum_{s \in (N(c) \setminus T)} y_s - 1, e^{-\eps})$. The former noise already yields $\eps$-DP as desired. 
\end{proof}

\subsection{Lower Bound}

For a bipartite graph $G = (S, C, E)$, we define a $\bt$-packing as a pair $C^{*} \subseteq C$ and $(T_c)_{c \in C^{*}}$ such that (i) $N(c) \setminus T_c$ are disjoint for all $c \in C^{*}$ and (ii) $|T_c| \leq t_c$. The size of the packing is $|C^{*}|$. We use $\optp^{\bt}$ to denote the largest size of $\bt$-packing for graph $G$.

Note that, when $\bt = \bzero$, $\bt$-packing coincides with the standard notion of set packing.

Firstly, we show that $\bt$-packing serves a crucial role in the lower bound of binary summation in the $\bt$-robust $\eps$-TDP model.

\begin{theorem}
Any $\bt$-robust $1$-TDP mechanism for binary summation must have MSE at least $\Omega\left(\sqrt{\optp^{\bt}}\right)$.
\end{theorem}

\begin{proof}[Proof Sketch]
Let $(C^{*}, (T_c)_{c \in C^{*}})$ be the $\bt$-packing of size $\optp^{\bt}$. We will argue that any $\bt$-robust 1-TDP mechanism $P$ for binary summation can be used to solve the same task (with the same error) in the local model with $n = \optp^{\bt}$ users; the lower bound then following from the known lower bound of \cite{ChanSS12}\footnote{See also \cite[Theorem 9.3]{Vadhan17} which restates this lower bound in local DP terminologies.}.

Suppose we are in the local DP model with $n = \optp^{\bt}$ users. We associate each user $i \in [n]$ with a unique $c_i^{*} \in C^{*}$. All parties then simulate $P$ as follows:
\begin{itemize}
\item User $i \in [n - 1]$ runs the protocol as $c_i^{*}$ (with its own input) and $N(c_i^{*}) \setminus T_{c_i^{*}}$. 
\item User $n$ runs the protocol as the remaining users, with $x_c = 0$ for all $c \notin C^{*}$.
\end{itemize}
It is not hard to see that the $\bt$-robust 1-TDP guarantee ensures that the above protocol satisfies 1-local DP.
\end{proof}

\pasin{I'm only claiming the lower bound above for $\eps = 1$ because \cite{ChanSS12} lower bound does not increase with $O(1/\eps)$. Needs to find a reference for that...}

Although we are not aware in general how large the gap between our upper and lower bounds are, we can show the following \emph{bi-criteria} result, that the uppper bound is not much larger than the lower bound \emph{when we increase $\bt$ slightly}. This is stated and proved below. 

We write $\lceil \eta \cdot \bt \rceil$ for some $\eta > 0$ as a shorthand for the vector $(\lceil \eta \cdot t_c\rceil)_{c \in C^{*}}$.

\begin{theorem}
For any $\alpha, \beta \in (0, 1)$, if $t_c \geq \beta \cdot \deg(c)$ for all $c \in C$, we have $\optp^{\lceil (1 + \alpha)\bt \rceil} \geq \Omega_{\alpha, \beta}(\optlp^{\bt})$.
\end{theorem}

\pasin{Note that the condition $t_c \geq \beta \cdot \deg(c)$ is required. Otherwise, we could set $t_c = 0$ which would falsify the inequality.}

\begin{proof}[Proof Sketch]
We will write $\bt'$ as a shorthand for $\lceil (1 + \alpha) \bt \rceil$.

We claim that there $\optp^{\bt'} \geq \gamma \cdot \optlp^{\bt}$ for $\gamma = \frac{\alpha\beta}{4}$. To prove this, first observe that LP duality implies that $\optlp^{\bt}$ is also equal to the optimal of the following LP:
\begin{align} \label{eq:dual-lp-robust}
&\max \sum_{c \in C, T \in \binom{N(c)}{t_c}} w_{c, T} \\
&\text{s.t.} \sum_{c \in C, T \in \binom{N(c)}{t_c} \atop (N(c) \setminus T) \ni s} w_{c, T} \leq 1 &\forall s \in S \label{eq:dual-sum-const} \\
& \qquad 0 \leq w_{c, T} \leq 1 &\forall c \in C, T \in \binom{N(c)}{t_c}. \nonumber
\end{align}
Note that, for $\bt = \bzero$, this is exactly the LP for the set packing problem (which has large ingrality gap).

Given an optimal solution $w_{s, c}$ to the dual LP \eqref{eq:dual-lp-robust}, we construct $\bt'$-packing as follows:
\begin{itemize}
\item First, use randomized rounding we include each $(c, T)$ in the set $R^0$ with probability $2\gamma \cdot w_{c, T}$. 
\item Next, we filter elements in $R^0$ to create $R^1$ where $R^1$ only includes $(c, T)$ such that
\begin{align*}
\left|\bigcup_{(c', T') \in (R^0 \setminus \{(c, T)\})} (N(c) \cap T')\right| \leq \alpha \cdot t_c. 
\end{align*}
\item Finally, we construct $R^2$ by, for each $(c, T) \in R^1$, add $\left(c, \bigcup_{(c', T') \in R^1} (N(c) \cap T')\right)$ to $R^2$.
\end{itemize}
It is simple to see that $R^2$ is a valid $\bt'$-packing. Thus, we are only left to argue that it has a large size. To do so, first observe that
\begin{align*}
\E[|R_2|] &= \E[|R_1|] \\
&= \sum_{c \in C, T \in \binom{N(c)}{t_c}} \Pr[(c, T) \in R_1] \\
&= \sum_{c \in C, T \in \binom{N(c)}{t_c}} \Pr[(c, T) \in R_0]\Pr[(c, T) \in R_1 \mid (c, T) \in R_0] \\
&= \sum_{c \in C, T \in \binom{N(c)}{t_c}} (2\gamma \cdot w_{c, T}) \cdot \Pr[(c, T) \in R_1 \mid (c, T) \in R_0].
\end{align*}
To bound $\Pr[(c, T) \in R_1 \mid (c, T) \in R_0]$, note that from our procedure, we have
\begin{align*}
\Pr[(c, T) \in R_1 \mid (c, T) \in R_0] &= \Pr\left[\left|\bigcup_{(c', T') \in (R^0 \setminus \{(c, T)\})} (N(c) \cap T')\right| \leq \alpha \cdot t_c\right] \\
&= 1 - \Pr\left[\left|\bigcup_{(c', T') \in (R^0 \setminus \{(c, T)\})} (N(c) \cap T')\right| > \alpha \cdot t_c\right] \\
&\geq 1 - \frac{\E\left[\left|\bigcup_{(c', T') \in (R^0 \setminus \{(c, T)\})} (N(c) \cap T')\right|\right]}{\alpha \cdot t_c} \\
&=  1 - \frac{\sum_{s \in N(c)} \Pr\left[s \in \bigcup_{(c', T') \in (R^0 \setminus \{(c, T)\})} T'\right]}{\alpha \cdot t_c} \\
&\geq 1 - \frac{\sum_{s \in N(c)} \sum_{c \in C, T \in \binom{N(c)}{t_c} \atop (N(c) \setminus T) \ni s} 2\gamma \cdot w_{c, T} }{\alpha \cdot t_c} \\
&\overset{\eqref{eq:dual-sum-const}}{\leq}  1 - \frac{2\gamma \cdot \deg(c)}{\alpha \cdot t_c} \\
&\geq 1/2,
\end{align*}
where the first inequality is from the Markov inequality and the last inequality is from our choice of $\gamma$ and from $t_c \geq \beta \deg(c)$.

Combining the above two sequence of inequalities, we get
\begin{align*}
\E[|R_2|] &\geq \sum_{c \in C, T \in \binom{N(c)}{t_c}} \gamma \cdot w_{c, T} = \gamma \cdot \optlp^{\bt},
\end{align*}
which concludes the proof.
\end{proof}
